Encoder-Decoder Framework for Interactive Free Verses with Generation with Controllable High-Quality Rhyming

Composing poetry or lyrics involves several creative factors, but a challenging aspect of generation is the adherence to a more or less strict metric and rhyming pattern. To address this challenge specifically, previous work on the task has mainly focused on reverse language modeling, which brings the critical selection of each rhyming word to the forefront of each verse. On the other hand, reversing the word order requires that models be trained from scratch with this task-specific goal and cannot take advantage of transfer learning from a Pretrained Language Model (PLM). We propose a novel fine-tuning approach that prepends the rhyming word at the start of each lyric, which allows the critical rhyming decision to be made before the model commits to the content of the lyric (as during reverse language modeling), but maintains compatibility with the word order of regular PLMs as the lyric itself is still generated in left-to-right order. We conducted extensive experiments to compare this fine-tuning against the current state-of-the-art strategies for rhyming, finding that our approach generates more readable text and better rhyming capabilities. Furthermore, we furnish a high-quality dataset in English and 12 other languages, analyse the approach's feasibility in a multilingual context, provide extensive experimental results shedding light on good and bad practices for lyrics generation, and propose metrics to compare methods in the future.

==> tables/multilingual_example1.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{\columnwidth}}
        \toprule
        \text{[Input]}\\
        <title>  Corazonado\\
        <artist> Ricky Martin\\
        <lang>   spanish\\
        <schema> AAAA\\
        <genre>  Latinsoft, desire\\
        \\
        \text{[Generation]}\\
        Cuanto tiempo esperaba para recuperar este amor\\
        De las ganas de matar el dolor\\
        Que te había dado alguna vez en el calor\\
        Y yo le pido por favor\\
        \\
        \text{[Gold]}\\
        Yo te ame\\
        De veras que te ame,\\
        Yo te ame,\\
        Te lo juro que te ame.\\
        \bottomrule
    \end{tabular}
    \caption{Example of a paragraph output from the multilingual model. }
    \label{tab:the_river_full}
\end{table}

==> tables/multilingual_example_new_1.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{\columnwidth}}
        \toprule
        \text{[Input]}\\
        <title> Lovecrimes\\
        <artist> Frank Ocean\\
        <lang> english\\
        <schema> ABACDEFG\\
        <genre>  R&B\\
        <topics> get, nigga, shit, bitch, ain, ass,yo, niggas, hit\\
        \\
        \text{[Generation]}\\
        generation
        I was a fool, I spent my life in the last time\\
        But, don't you think that I'm yours, when she was mine?\\
        She took my time, she did my love crime\\
        Now I know\\
        You got the keys to my heart, baby, girl, you\\
        Then we got love\\
        We're sorry, but, it wasn'ting what we do\\
        To make you feel like you love me\\
        \\
        \text{[Gold]}\\
        Eh, murder, murder, murder she wrote\\
        love crimes, love crimes\\
        Murder, murder, murder she wrote\\
        Love crimes, love crimes\\
        Oh, yeah, yeah\\
        Murder, murder, murder she wrote\\
        Love crimes, love crimes\\
        Oh, yeah, yeah\\
        \bottomrule
    \end{tabular}
    \caption{Example of a paragraph output from the multilingual model. The topics come from the LDA topic modeling done in Wasabi dataset}
    \label{tab:the_river_full}
\end{table}

==> tables/the_river.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{p{\columnwidth}}
        \toprule
        A: river <sep> That night we went down to the river \\
        B: dive <sep> And into the river we’d dive \\
        B: ride <sep> Oh, down to the river we did ride.\\
        \bottomrule
    \end{tabular}
    \caption{"The River" by Bruce Springsteen.}
    \label{tab:the_river}
\end{table}

==> tables/wish_you_were_here_verses.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{\columnwidth}}
        \toprule
        So, so you think you can tell\\
        Heaven from hell?\\
        Blue skies from pain?\\
        Can you tell a green field\\
        From a cold steel rail?\\
        A smile from a veil?\\
        Do you think you can tell?\\
        \bottomrule
    \end{tabular}
    \caption{"Wish you were here" by Pink Floyd, with schema \texttt{AABCDDA}}
    \label{tab:wish_you_were_here}
\end{table}
